Multi-Scale Vision Longformer: A New Vision Transformer for High-Resolution Image Encoding

This paper presents a new Vision Transformer (ViT) architecture Multi-Scale Vision Longformer, which significantly enhances the ViT of \cite{dosovitskiy2020image} for encoding high-resolution images using two techniques. The first is the multi-scale model structure, which provides image encodings at multiple scales with manageable computational cost. The second is the attention mechanism of vision Longformer, which is a variant of Longformer \cite{beltagy2020longformer}, originally developed for natural language processing, and achieves a linear complexity w.r.t. the number of input tokens. A comprehensive empirical study shows that the new ViT significantly outperforms several strong baselines, including the existing ViT models and their ResNet counterparts, and the Pyramid Vision Transformer from a concurrent work \cite{wang2021pyramid}, on a range of vision tasks, including image classification, object detection, and segmentation. The models and source code are released at \url{https://github.com/microsoft/vision-longformer}.

==> app_corrections.tex <==
\section{Corrections and Modifications of the main paper}
While we are preparing this supplementary material, we identified several typos in the paper. Therefore, we made the following corrections and modifications the main paper.
\begin{itemize}
    \item The model configuration of Medium-W and Base-W in Table~\ref{tab:model_arch} has some typo. It's corrected in the updated Table~\ref{tab:model_arch}.
    \item The number of parameters in Table~\ref{tab:attention_maskrcnn} has some typos for Global and Performer. It's corrected in the updated Table~\ref{tab:attention_maskrcnn}.
    \item As mentioned in the main paper, we experimented Spatial Reduction Attention in our multi-scale vision transformer framework with Spatial Reduction ratios $R_1=16, R_2=8,R_3=4, R_4=2$ (two times more downsizing from that in PVT~\cite{wang2021pyramid}, short as SRA/64), to make its memory usage comparable with other efficient attention mechanisms under the same model size. This more aggressive downsizing introduces more parameters due to doubling the kernel size of the convolutional projection layer, and also results in worser performance in ImageNet classification and COCO detection tasks. We add one set of experiments with Spatial Reduction ratios $R_1=8, R_2=4,R_3=2, R_4=1$ (the same with that in PVT~\cite{wang2021pyramid}, short as SRA/32), and report its ImageNet classification results in the updated Table~\ref{tab:eff_attns} and COCO detection results in the updated Table~\ref{tab:attention_maskrcnn}. We can see that SRA/32 has much better performance than SRA/64, but still has a gap from our Vision Longformer. 
\end{itemize}

==> app_deit_vis.tex <==
\section{Visualization of DeiT's attention maps to validate the inductive bias in Vision Longformer}
% \begin{figure}[t!]
% \includegraphics[width=0.48\textwidth]{figs/imange_val002.png}
% \caption{Image from ImageNet validation set.}
% \label{fig:deit_pic}
% \end{figure}
We visualize the attention maps from DeiT's pretrained models to argue that the "local attention + global memory" mechanism in Vision Longformer is a reasonable inductive bias for vision transformers. More specifically, we take the pretrained DeiT-Tiny model from \url{https://dl.fbaipublicfiles.com/deit/deit_tiny_patch16_224-a1311bcf.pth}, infer it on images from ImageNet validation set, and display its attention maps of the first attention block in Figure~\ref{fig:deit_tiny_block0_head0}, \ref{fig:deit_tiny_block0_head1} and \ref{fig:deit_tiny_block0_head2}, for head 0, head 1 and head 2, respectively. 

In Figure~\ref{fig:deit_tiny_block0_head0}, the attention map of head 0 is just like the 2-D convolution, focusing on neighboring patches. There are also relative large weights on the CLS token. In Figure~\ref{fig:deit_tiny_block0_head2}, the attention map of head 0 is just like the ``global memory" mechanism, with every local token attends to the global CLS token. Each local token also attends to itself, like ``local attention" with window size 1. In Figure~\ref{fig:deit_tiny_block0_head1}, the attention map of head 1 seems to be global, with large attention scores on visually similar patches (i.e., the dog's white fur, the gray wall).

These three attention patterns for these three heads are consistent for different images. For other DeiT pretrained models (like DeiT-Small and DeiT-Base), their attention maps in the first attention block can also be classified into these three attention patterns. Longformer exactly captures the "local attention" and the "global memory" patterns, and may introduce some information loss for the ``global-similarity" pattern.  In  comparison  with  the full attention, the Vision Longformer attention does not lead to any accuracy drop in low-resolution ImageNet classification problem (Table~\ref{tab:flatvsmultiscale}) and leads to small accuracy drop in high-resolution Object Detection/Segmentation tasks (Table~\ref{tab:attention_maskrcnn}).

\begin{figure*}[t!]
\includegraphics[width=0.25\textwidth]{figs/imange_val002.png}\\
\includegraphics[width=0.98\textwidth]{figs/block0_head0.png}
\caption{Attention map of DeiT-Tiny at Block 0, head 0. This head's attention map has exactly the "local attention + global memory" pattern in Vision Longformer, with more emphasis on the "local attention". The $(i,j)$ subplot shows the attention map of the local token $(2*i, 2*j)$ as query. Each attention map $A$ is a matrix of size $15 \times 14$, where $A[1:15, 0:14]$ is the attention scores to the $14\times 14$ local tokens and $A[0,13]$ (top-right corner) shows the attention score to the CLS token. $A[0,0:13]$ are zeros.}
\label{fig:deit_tiny_block0_head0}
\end{figure*}

\begin{figure*}[t!]
\includegraphics[width=0.25\textwidth]{figs/imange_val002.png}\\
\includegraphics[width=0.98\textwidth]{figs/block0_head1.png}
\caption{DeiT-Tiny: Block 0, head 1. This head's attention map seems to be global, with large attention scores on visually similar patches (i.e., the dog's white fur, the gray wall). The $(i,j)$ subplot shows the attention map of the local token $(2*i, 2*j)$ as query. Each attention map $A$ is a matrix of size $15 \times 14$, where $A[1:15, 0:14]$ is the attention scores to the $14\times 14$ local tokens and $A[0,13]$ (top-right corner) shows the attention score to the CLS token. $A[0,0:13]$ are zeros.}
\label{fig:deit_tiny_block0_head1}
\end{figure*}

\begin{figure*}[t!]
\includegraphics[width=0.25\textwidth]{figs/imange_val002.png}\\
\includegraphics[width=0.98\textwidth]{figs/block0_head2.png}
\caption{DeiT-Tiny: Block 0, head 2. This head's attention map has exactly the "local attention + global memory" pattern in Vision Longformer, with more emphasis on the "global memory". The $(i,j)$ subplot shows the attention map of the local token $(2*i, 2*j)$ as query. Each attention map $A$ is a matrix of size $15 \times 14$, where $A[1:15, 0:14]$ is the attention scores to the $14\times 14$ local tokens and $A[0,13]$ (top-right corner) shows the attention score to the CLS token. $A[0,0:13]$ are zeros.}
\label{fig:deit_tiny_block0_head2}
\end{figure*}

==> cls_relative_app.tex <==
\section{Classification results with relative positional bias}

\begin{table}[ht]
\begin{center}
% \scriptsize
\footnotesize
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c}
\toprule
Model & \#Params (M) & GFLOPs & Top-1 (\%) \\
\midrule
R18 & 11.7 & 1.8 & 69.8 \\
DeiT-Tiny/16\cite{touvron2020training} & 5.7 & 1.3 & 72.2 \\
\rowcolor{Graylight} 
\vil-Tiny & 6.7 & 1.3 & 76.7 \\
\midrule
R50 & 25.6 & 4.1 & 78.5 \\
DeiT-Small/16\cite{touvron2020training} & 22.1 & 4.6 & 79.9 \\
Swin-Tiny & 28 & 4.5 & 81.2 \\
\rowcolor{Graylight} 
\vil-Small & 24.6 & 5.1 & 82.4 \\
\midrule
R101 & 44.7 & 7.9 & 79.8 \\
ViT-Small/16\cite{dosovitskiy2020image} & 48.8 & 9.9 & 80.8 \\
Swin-Small & 50 & 8.7 & 83.2 \\
\rowcolor{Graylight} 
\vil-Medium & 39.7 & 9.1 & 83.5 \\
\midrule
X101-64x4d & 83.5 & 15.6 & 81.5 \\
ViT-Base/16\cite{dosovitskiy2020image} & 86.6 & 17.6 & 77.9 \\
DeiT-Base/16\cite{touvron2020training} & 86.6 & 17.6 & 81.8 \\
Swin-Base & 88 & 15.4 & 83.5 \\
\rowcolor{Graylight} 
\vil-Base & 55.7 & 13.4 & 83.7 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Number of paramers, FLOPS and ImageNet accuracy. Trained on ImageNet-1K with image size 224. Our \vil~~models are highlighted with gray background.}
\label{tab:cls_relative_1k}
\end{table}


\begin{table}[ht]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c}
\toprule
\multirow{2}{*}{Model} & \#Params & FLOPs & IN-21K & JFT-300M \\
& (M) & (G) & Top-1 & Top-1 \\
\midrule
BiT-152x4 \cite{kolesnikov2019big} & 928 & 837 & 85.4 & 87.54 \\
\midrule
ViT-Base/16\cite{dosovitskiy2020image} & 86.6 & 49.3 & 84.0 & 84.15 \\
ViT-Large/16\cite{dosovitskiy2020image} & 307 & 191.1 & 85.2 & 87.12 \\
ViT-Huge/14\cite{dosovitskiy2020image} & 632 & 474 & -- & 88.55 \\
\midrule
Swin-Base & 88 & 47.1 & 86.4 & -- \\
Swin-Large & 197 & 103.9 & 87.3 & --\\
\midrule
\rowcolor{Graylight} 
\vil-Medium & 39.7 & 29.4 & 85.7 & --\\
\rowcolor{Graylight} 
\vil-Base & 55.7 & 45.3 & 86.2 & --\\
\rowcolor{Graylight} 
\vil-Large & 220 & 113 & ?? & ?? \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Pretained on ImageNet-21K ( IN-21K) or JFT-300M with image size 224 and Finetuned on ImageNet-1K with image size 384, except BiT-M~\cite{kolesnikov2019big} fine-tuned with image size 480. Our \vil~~models are highlighted with gray background.}
\label{tab:cls_relative_22k}
\end{table}

==> detection_exps_3xms.tex <==
\begin{table*}[ht]
\begin{center}
% \scriptsize
% \footnotesize
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c}
\toprule
Backbone & \#Params(M) & GFLOPs & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$\\
\midrule
ResNet18 & 21.3 & 190.33 & 35.4 & 53.9 & 37.6 & 19.5 & 38.2 & 46.8 \\
PVT-Tiny\cite{wang2021pyramid} & 23.0 & n/a & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\
% https://ml.azure.com/job/msrhyper/msr-lab-dell-hyper/3176334eebb96afd4f503607c9cfcb41
% max_mem: 7167M
\vil-Tiny & 16.64 & 171.91 & 40.7 & 61.2 & 43.2 & 26.4 & 43.9 & 53.6 \\
\midrule
ResNet50 & 37.7 & 239.32 & 39.0 & 58.4 & 41.8 & 22.4 & 42.8 & 51.6 \\
PVT-Small\cite{wang2021pyramid} & 34.2 & n/a & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2 \\
% https://ml.azure.com/job/resrchvc/Az-SEA-V100-16GB/99a9b0716fc6b560afbb690bbcc4667a
% 1300M
\vil-Small & 35.68 & 252.21 & 42.9 & 63.8 & 45.6 & 27.8 & 46.4 & 56.3 \\
\midrule
ResNet101 & 56.7 & 319.07 & 40.9 & 60.1 & 44.0 & 23.7 & 45.0 & 53.8 \\
ResNeXt101-32x4d & 56.4 & 319.07 & 41.4 & 61.0 & 44.3 & 23.9 & 45.5 & 53.7 \\
PVT-Medium\cite{wang2021pyramid} & 53.9 & n/a & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\
% https://ml.azure.com/job/resrchvc/lab-rr1-v100-32gb-4/ccbb8fc7e82205e2246ab2d5655690ee
% max_mem: 20530M
\vil-Medium & 50.77 & 338.93 & 43.7 & 64.6 & 46.4 & 27.9 & 47.1 & 56.9 \\
\midrule
ResNeXt101-64x4d & 95.5 & 483.59 & 41.8 & 61.5 & 44.4 & 25.2 & 45.4 & 54.6 \\
PVT-Large\cite{wang2021pyramid} & 71.1 & n/a & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
% 
% max_mem: 21456M
\vil-Base & 66.74 & 443.0 & 44.7 & 65.5 & 47.6 & 29.9 & 48.0 & 58.1 \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\caption{Object detection performance on the COCO val2017 with RetinaNet trained with ``3$\times$+MS" scheduling. “\#Params” refers to parameter number. The GFLOPs for PVT architecture are not available. \vil models are pretrained on ImageNet-1K. }
\label{tab:retinanet_comp_det_3xms}
\vspace{-2mm}
\end{table*}

\begin{table*}[ht]
\begin{center}
% \scriptsize
% \footnotesize
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c}
\toprule
Backbone & \#Params(M) & GFLOPs & $AP^b$ & $AP^b_{50}$ & $AP^b_{75}$ & $AP^m$ & $AP^m_{50}$ & $AP^m_{75}$\\
\midrule
ResNet18 & 31.2 & 131.03 & 36.9 & 57.1 & 40.0 & 33.6 & 53.9 & 35.7
 \\
PVT-Tiny\cite{wang2021pyramid} & 32.9 & n/a & 39.8 & 62.2 & 43.0 & 37.4 & 59.3 & 39.9 \\
\vil-Tiny & 26.9 & 94.3 & 41.2 & 63.0 & 44.7 & 37.9 & 59.8 & 40.6 \\

% https://ml.azure.com/job/resrchvc/az-eus-v100-16gb-2/36255ae140052573c1ea521dacf90440
\midrule
ResNet50 & 44.2 & 180.0 & 41.0 & 61.7 & 44.9 & 37.1 & 58.4 & 40.1 \\
PVT-Small\cite{wang2021pyramid} & 44.1 & n/a & 43.0 & 65.3 & 46.9 & 39.9 & 62.5 & 42.8 \\
\vil-Small & 45.0 & 174.3 & 43.4 & 64.9 & 47.0 & 39.6 & 62.1 & 42.4 \\
\midrule
ResNet101 & 63.2 & 259.77  & 42.8 & 63.2 & 47.1 & 38.5 & 60.1 & 41.3 \\
ResNeXt101-32x4d & 62.8 & 259.77 & 44.0 & 64.4 & 48.0 & 39.2 & 61.4 & 41.9 \\
PVT-Medium\cite{wang2021pyramid} & 63.9 & n/a & 44.2 & 66.0 & 48.2 & 40.5 & 63.1 & 43.5 \\
\vil-Medium & 60.1 & 261.1 & 44.6 & 66.3 & 48.5 & 40.7 & 63.8 & 43.7 \\
% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/13f2aa35db37c75657fb997ad0be18b8
\midrule
ResNeXt101-64x4d & 101.9 & 424.29 & 44.4 & 64.9 & 48.8 & 39.7 & 61.9 & 42.6 \\
PVT-Large\cite{wang2021pyramid} & 81.0 & n/a & 44.5 & 66.0 & 48.3 & 40.7 & 63.4 & 43.7 \\
\vil-Base & 76.1 & 365.1 & 45.7 & 67.2 & 49.9 & 41.3 & 64.4 & 44.5 \\
% msvit_maskrcnn_fpn_3xms_base_lr8e-5_wd015
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\caption{Object detection and instance segmentation performance on the COCO val2017 with Mask R-CNN trained with ``3$\times$+MS" scheduling. “\#Params” refers to parameter number. Similarly to RetinaNet, the GFLOPs for PVT architecture are not available. \vil models are pretrained on ImageNet-1K.}
\label{tab:maskrcnn_comp_det_3xms}
\vspace{-2mm}
\end{table*}


==> detection_exps_all.tex <==
\begin{table*}[ht]
\begin{center}
% \scriptsize
% \footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Backbone} & \#Params & FLOPs & \multicolumn{6}{c|}{RetinaNet 1x schedule} & \multicolumn{6}{c}{RetinaNet 3x + MS schedule}\\
& (M) & (G) & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
\midrule
ResNet18 & 21.3 & 190.33 & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2 & 35.4 & 53.9 & 37.6 & 19.5 & 38.2 & 46.8 \\
PVT-Tiny\cite{wang2021pyramid} & 23.0 & n/a & 36.7 & 56.9 & 38.9 & 22.6 & 38.8 & 50.0 & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\
% https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-retina_msvit_tiny_lr1e-4_qkvbiastrue_scus-trainval_retinanet_with_msvit_widemedim_lr1e-4_wd0_1_bsz16-160385b0?wsid=/subscriptions/8d7c0a6f-7c2e-4e4b-becf-f9ee95433147/resourcegroups/Image_Languge_Pretraining-aml/workspaces/Image_Languge_Pretraining-aml
% max_mem: 7167M
\rowcolor{Graylight} 
\vil-Tiny & 16.64 & 182.7 & 38.8 & 59.0 & 41.3 & 23.8 & 41.5 & 51.8 & 40.7 & 61.2 & 43.2 & 26.4 & 43.9 & 53.6 \\
\midrule
ResNet50 & 37.7 & 239.32 & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8 & 39.0 & 58.4 & 41.8 & 22.4 & 42.8 & 51.6 \\
PVT-Small\cite{wang2021pyramid} & 34.2 & n/a & 40.4 & 61.3 & 43.0 & 25.0 & 42.9 & 55.7 & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2\\
% https://ml.azure.com/experiments/msvit_det-9f976a33/runs/msvit_det-9f976a33-retina_msvit_small_lr1e-4_smallwd_qkvbiastrue-trainval_retinanet_with_msvit_small_wd5e-2-2049f92b?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/researchvc-sea/workspaces/resrchvc-sea
% 1300M
\rowcolor{Graylight} 
\vil-Small & 35.68 & 254.8 & 41.6 & 62.5 & 44.1 & 24.9 & 44.6 & 56.2 & 42.9 & 63.8 & 45.6 & 27.8 & 46.4 & 56.3 \\
\midrule
ResNet101 & 56.7 & 319.07 & 38.5 & 57.8 & 41.2 & 21.4 & 42.6 & 51.1 & 40.9 & 60.1 & 44.0 & 23.7 & 45.0 & 53.8 \\
ResNeXt101-32x4d & 56.4 & 319.07 & 39.9 & 59.6 & 42.7 & 22.3 & 44.2 & 52.5 & 41.4 & 61.0 & 44.3 & 23.9 & 45.5 & 53.7 \\
PVT-Medium\cite{wang2021pyramid} & 53.9 & n/a & 41.9 & 63.1 & 44.3 & 25.0 & 44.9 & 57.6 & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\
% https://ml.azure.com/job/Image_Languge_Pretraining/az-scus-v100-2/111e3a7b1cf47eb9330abb66817e3bfc
% max_mem: 20530M
\rowcolor{Graylight} 
\vil-Medium & 50.77 & 330.4 & 42.9 & 64.0 & 45.4 & 27.0 & 46.1 & 57.2 & 43.7 & 64.6 & 46.4 & 27.9 & 47.1 & 56.9 \\
\midrule
ResNeXt101-64x4d & 95.5 & 483.59 & 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0 & 41.8 & 61.5 & 44.4 & 25.2 & 45.4 & 54.6 \\
PVT-Large\cite{wang2021pyramid} & 71.1 & n/a & 42.6 & 63.7 & 45.4 & 25.8 & 46.0 & 58.4 & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
% https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-retina_msvit_base_lr8e-5_qkvbiastrue-trainval_retinanet_with_msvit_deepbase_lr8e-5_wd0_15-2c10da1b?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/msrhyperVC/workspaces/msrhyper
% max_mem: 21456M
\rowcolor{Graylight} 
\vil-Base & 66.74 & 420.9 & 44.3 & 65.5 & 47.1 & 28.9 & 47.9 & 58.3 & 44.7 & 65.5 & 47.6 & 29.9 & 48.0 & 58.1 \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{Object detection performance on the COCO val2017 with RetinaNet. The FLOPs (G) are measured at resolution $800\times 1333$, and FLOPs for PVT architecture are not available. Our \vil~~models are pre-trained on ImageNet-1K and highlighted with gray background.}
\label{tab:retinanet_comp_det}
\vspace{-2mm}
\end{table*}

\begin{table*}[ht]
\begin{center}
% \scriptsize
% \footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Backbone} & \#Params & FLOPs & \multicolumn{6}{c|}{Mask R-CNN 1x schedule} & \multicolumn{6}{c}{Mask R-CNN 3x + MS schedule}\\
 & (M) & (G) & $AP^b$ & $AP^b_{50}$ & $AP^b_{75}$ & $AP^m$ & $AP^m_{50}$ & $AP^m_{75}$ & $AP^b$ & $AP^b_{50}$ & $AP^b_{75}$ & $AP^m$ & $AP^m_{50}$ & $AP^m_{75}$ \\
\midrule
ResNet18 & 31.2 & 131.03 & 34.0 & 54.0 & 36.7 & 31.2 & 51.0 & 32.7 & 36.9 & 57.1 & 40.0 & 33.6 & 53.9 & 35.7\\
PVT-Tiny\cite{wang2021pyramid} & 32.9 & n/a & 36.7 & 59.2 & 39.3 & 35.1 & 56.7 & 37.3 & 39.8 & 62.2 & 43.0 & 37.4 & 59.3 & 39.9 \\
\rowcolor{Graylight} 
\vil-Tiny & 26.9 & 145.6 & 38.7 & 61.1 & 41.3 & 36.2 & 58.3 & 38.2 & 41.2 & 63.0 & 44.7 & 37.9 & 59.8 & 40.6 \\
% https://ml.azure.com/job/resrchvc/az-eus-v100-16gb-2/36255ae140052573c1ea521dacf90440
\midrule
ResNet50 & 44.2 & 180.0 & 38.0 & 58.6 & 41.4 & 34.4 & 55.1 & 36.7 & 41.0 & 61.7 & 44.9 & 37.1 & 58.4 & 40.1 \\
PVT-Small\cite{wang2021pyramid} & 44.1 & n/a & 40.4 & 62.9 & 43.8 & 37.8 & 60.1 & 40.3 & 43.0 & 65.3 & 46.9 & 39.9 & 62.5 & 42.8 \\
\rowcolor{Graylight} 
\vil-Small & 45.0 & 218.3 & 41.8 & 64.1 & 45.1 & 38.5 & 61.1 & 41.4 & 43.4 & 64.9 & 47.0 & 39.6 & 62.1 & 42.4 \\
% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/1378be65b7aa1c206bfa74226a38c86a
% exp: https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/6c2b53df6881b2866f3bfaf056b52c6f
% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/e37f414585c5d86cac795cab230d1ead
\midrule
ResNet101 & 63.2 & 259.77  & 40.4 & 61.1 & 44.2 & 36.4 & 57.7 & 38.8 & 42.8 & 63.2 & 47.1 & 38.5 & 60.1 & 41.3 \\
ResNeXt101-32x4d & 62.8 & 259.77 & 41.9 & 62.5 & 45.9 & 37.5 & 59.4 & 40.2 & 44.0 & 64.4 & 48.0 & 39.2 & 61.4 & 41.9 \\
PVT-Medium\cite{wang2021pyramid} & 63.9 & n/a & 42.0 & 64.4 & 45.6 & 39.0 & 61.6 & 42.1 & 44.2 & 66.0 & 48.2 & 40.5 & 63.1 & 43.5 \\
\rowcolor{Graylight} 
\vil-Medium & 60.1 & 293.8 & 43.4 & 65.9 & 47.0 & 39.7 & 62.8 & 42.1 & 44.6 & 66.3 & 48.5 & 40.7 & 63.8 & 43.7 \\
% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/13f2aa35db37c75657fb997ad0be18b8
\midrule
ResNeXt101-64x4d & 101.9 & 424.29 & 42.8 & 63.8 & 47.3 & 38.4 & 60.6 & 41.3 & 44.4 & 64.9 & 48.8 & 39.7 & 61.9 & 42.6 \\
PVT-Large\cite{wang2021pyramid} & 81.0 & n/a & 42.9 & 65.0 & 46.6 & 39.5 & 61.9 & 42.5 & 44.5 & 66.0 & 48.3 & 40.7 & 63.4 & 43.7 \\
\rowcolor{Graylight} 
\vil-Base & 76.1 & 384.4 & 45.1 & 67.2 & 49.3 & 41.0 & 64.3 & 44.2 & 45.7 & 67.2 & 49.9 & 41.3 & 64.4 & 44.5 \\
% https://ml.azure.com/job/msrhyper/msr-lab-hyper-dgx2/ad92391242af8a3560c8c6be6f57c732
% https://ml.azure.com/job/msrhyper/msr-lab-hyper-dgx2/49f8a2e7359ef8a071f64125640f176d
% https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-maskrcnn_msvit_base_lr1e-4_largewd_qkvbiastrue-trainval_maskrcnn_with_msvit_large_sparse_attn_avg_token_no_freeze_backbonelr1_0_1e-4_wd1e-1-e47153d1?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/msrhyperVC/workspaces/msrhyper
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{Object detection and instance segmentation performance on the COCO val2017 with Mask R-CNN. The FLOPs (G) are measured at resolution $800\times 1333$, and FLOPs for PVT architecture are not available. Our \vil~~models are pre-trained on ImageNet-1K and highlighted with gray background.}
\label{tab:maskrcnn_comp_det}
\vspace{-3mm}
\end{table*}

